Scene Style Text Editing

In this work, we propose a task called "Scene Style Text Editing (SSTE)", changing the text content as well as the text style of the source image while keeping the original text scene. Existing methods neglect to fine-grained adjust the style of the foreground text, such as its rotation angle, color, and font type. To tackle this task, we propose a quadruple framework named "QuadNet" to embed and adjust foreground text styles in the latent feature space. Specifically, QuadNet consists of four parts, namely background inpainting, style encoder, content encoder, and fusion generator. The background inpainting erases the source text content and recovers the appropriate background with a highly authentic texture. The style encoder extracts the style embedding of the foreground text. The content encoder provides target text representations in the latent feature space to implement the content edits. The fusion generator combines the information yielded from the mentioned parts and generates the rendered text images. Practically, our method is capable of performing promisingly on real-world datasets with merely string-level annotation. To the best of our knowledge, our work is the first to finely manipulate the foreground text content and style by deeply semantic editing in the latent feature space. Extensive experiments demonstrate that QuadNet has the ability to generate photo-realistic foreground text and avoid source text shadows in real-world scenes when editing text content.

==> figures/combination/real_scene.tex <==
\begin{figure*}[t]
\centering
\begin{minipage}{0.16\linewidth}
\centering
    Source Image
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/1f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
    New Content
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/0o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
 Source Image
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/3f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
 New Content
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/2o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
 Source Image
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/5f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
    \centering
    New Content
    \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/4o.jpg}
\end{minipage}


\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/7f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/6o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/9f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/8o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/59f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
    \centering
    \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/58o.jpg}
\end{minipage}



\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/13f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/12o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/57f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/56o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/17f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
    \centering
    \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/16o.jpg}
\end{minipage}


\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/19f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/18o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/21f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/20o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/23f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
    \centering
    \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/22o.jpg}
\end{minipage}


\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/25f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/24o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/27f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/26o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/29f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
    \centering
    \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/28o.jpg}
\end{minipage}


\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/31f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/30o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/55f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/54o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/35f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
    \centering
    \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/34o.jpg}
\end{minipage}



\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/37f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/36o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/39f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/38o.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
	\centering
	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/41f.jpg}
\end{minipage}
\begin{minipage}{0.16\linewidth}
    \centering
    \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/40o.jpg}
\end{minipage}

% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/43f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/42o.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/45f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/44o.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/47f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/46o.jpg}
% \end{minipage}

% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/49f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/48o.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/51f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/50o.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/53f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/52o.jpg}
% \end{minipage}

% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/55f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/54o.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/57f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/56o.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
% 	\centering
% 	\includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/59f.jpg}
% \end{minipage}
% \begin{minipage}{0.16\linewidth}
%     \centering
%     \includegraphics[width=1\linewidth, height=0.4\linewidth]{figures/RealScene/58o.jpg}
% \end{minipage}


\caption{Generated images by our QuadNet with new content: change the text content and keep the text style and background texture of the source image, which are drawn from real-world data.
}
\label{fig:real_scene}
\end{figure*}


==> figures/combination/z_t-SNE.tex <==
\begin{figure*}[t]
\centering 
\subfigure[$\mathbf {z}$ about rotate]{
\label{Fig.z.rotate}
\includegraphics[width=0.3\textwidth, trim=30 10 0 50]{figures/tsne/z/style_vector_rotate.png}}
\subfigure[$\mathbf {z}$ about font]{
\label{Fig.z.font}
\includegraphics[width=0.3\textwidth, trim=30 10 0 50]{figures/tsne/z/style_vector_font.png}}
\subfigure[$\mathbf {z}$ about color]{
\label{Fig.z.color}
\includegraphics[width=0.3\textwidth, trim=30 10 0 50]{figures/tsne/z/style_vector_color.png}}
\caption{t-SNE visualizations of $\mathbf{z}$ about text style attributes: 
corresponding to the three images in Figure \ref{fig.W_t-SNE}, $\mathbf {z}$ is not as distinguishable as the $\mathbf{w}^{i}$ with regard to attributes such as rotation angle, font, and color.}
\label{fig.z_t-SNE}
\end{figure*}

==> sections/6-Other.tex <==
\appendix

\section*{Ethical Statement}

There are no ethical issues.

\section*{Acknowledgments}

TODO
